An Efficient Private GPT Never Autoregressively Decodes

The wide deployment of the generative pre-trained transformer (GPT) has raised privacy concerns for both clients and servers. While cryptographic primitives can be employed for secure GPT inference to protect the privacy of both parties, they introduce considerable performance overhead.To accelerate secure inference, this study proposes a public decoding and secure verification approach that utilizes public GPT models, motivated by the observation that securely decoding one and multiple tokens takes a similar latency. The client uses the public model to generate a set of tokens, which are then securely verified by the private model for acceptance. The efficiency of our approach depends on the acceptance ratio of tokens proposed by the public model, which we improve from two aspects: (1) a private sampling protocol optimized for cryptographic primitives and (2) model alignment using knowledge distillation. Our approach improves the efficiency of secure decoding while maintaining the same level of privacy and generation quality as standard secure decoding. Experiments demonstrate a $2.1\times \sim 6.0\times$ speedup compared to standard decoding across three pairs of public-private models and different network conditions.

==> tex_files/Outline.tex <==




\section{Introduction}
GPT is popular, and using secure inference guarantees privacy of both client and server.

The common way includes optimizing the cryptographic protocols or modify the GPT to tailor the cryptographic primitives.

This work considers an orthogonal approach targeting secure inference scheme. We notice many powerful GPT models are publicly available. Although a private model are trained on a private dataset, the underlying rules of languages are not sensitive, and can be captured by those public model. If there is a proper way to separate the private and public parts of the private model, we can utilize the public model to assist the secure inference. 

However, to determine the privacy sensitivity of the GPT model is difficult due to its uninterpretable property.
Existing methods adopt finetune methods similar to LoRA. Only a small parts of parameters needs to be securely evaluated. However, this cannot benefit the nonlinear layers and has a restriction of base model selection.

This work proposes a new scheme to perform the secure inference: public drafting-then-private verification. There are two key observations that motivates the design of our techniques. First, the language pattern makes the decoding of some tokens easier so that public and private models produce same token. Second, we analyze the unique cost profile of MPC and find increasing the extreme small sequence length 1 almost  does not affect the latency.


Using our public drafting-then-private verification scheme, we propose two designs.
First, we design a private sampling protocol to make the output tokens keep identical as the private model. 
We have noticed that due to the different linguistic habits between the public model and the private model, draft words with the same meaning but expressed in different ways are rejected. Therefore, we align the linguistic habits of the public model with the private model through knowledge distillation, without compromising any privacy.

Our experiments on ...


\section{Preliminary}

\subsection{Secure Two-Party Inference}
\begin{itemize}
    \item The MLaaS scenario and privacy goal.
    \item The mechanism: how the linear and nonlinear layers are evaluated through cryptographic primitives.
    \item Building blocks: necessary background of secret sharing, HE, and OT.
\end{itemize}

\subsection{Decoding of the GPT}
\begin{itemize}
    \item Explain decoding and standard sampling of GPT.
\end{itemize}


\section{Motivations}
\subsection{Common Knowledge between Public and Private GPT}
\begin{itemize}
    \item The powerful publicly available GPT models.
    \item Public and private GPTs share basic language knowledge. Only the privacy regarding to the specific private dataset should be protected. Public parts can be used to assist secure inference.
    \item Difficulty of distinguish the privacy sensitivity and limitation of existng LoRA efforts.
\end{itemize}

\subsection{Insensitivity of Latency against the Sequence Length}
\begin{itemize}
    \item Introduce the observation.
    \item Analyzing reasons about computation time, transmission time, and one-way delay.
    \item A possible assistant way: public drafting, and then private verification
\end{itemize}


  


\section{Secure Inference through Public-Private GPT Collaboration }


\subsection{Secure Speculative Sampling Protocol}
\begin{itemize}
    \item The design makes improvements on naive translation.
    \item security analysis
\end{itemize}

\subsection{Aligning Public and Private GPT}
The realigned data are used to extract model weights.
\begin{itemize}
    \item The data collection for knowledge distillation, which does not use extra information.
    \item Loss function for the knowledge distillation.
\end{itemize}





\section{Evaluation}
\subsection{Accuracy of Speculative Sampling}

\subsection{Efficiency Comparison}

\section{Related Works}
See later sections.


\section{Conclusion}
\newpage
